A stencil scaling approach for accelerating matrix-free finite element implementations

We present a novel approach to fast on-the-fly low order finite element assembly for scalar elliptic partial differential equations of Darcy type with variable coefficients optimized for matrix-free implementations. Our approach introduces a new operator that is obtained by appropriately scaling the reference stiffness matrix from the constant coefficient case. Assuming sufficient regularity, an a priori analysis shows that solutions obtained by this approach are unique and have asymptotically optimal order convergence in the $H^1$- and the $L^2$-norm on hierarchical hybrid grids. For the pre-asymptotic regime, we present a local modification that guarantees uniform ellipticity of the operator. Cost considerations show that our novel approach requires roughly one third of the floating-point operations compared to a classical finite element assembly scheme employing nodal integration. Our theoretical considerations are illustrated by numerical tests that confirm the expectations with respect to accuracy and run-time. A large scale application with more than a hundred billion ($1.6\cdot10^{11}$) degrees of freedom executed on 14,310 compute cores demonstrates the efficiency of the new scaling approach.

==> scale.tex <==
\todo[inline]{this chapter should contain some run time results}

\todoSBinline{Das sind zwar noch keine large scale results, aber bei 32 Prozessoren beobachte ich
   fuer den divK Fall dass die Laufzeiten fuer einen V(3,3) Zyklus mit dem Scaling Ansatz um ca. den Faktor 
   2.5 schneller werden. Für den Poisson sieht es ähnlich aus.}
